Profitable Task Allocation in Mobile Cloud Computing

We propose a game theoretic framework for task allocation in mobile cloud computing that corresponds to offloading of compute tasks to a group of nearby mobile devices. Specifically, in our framework, a distributor node holds a multidimensional auction for allocating the tasks of a job among nearby mobile nodes based on their computational capabilities and also the cost of computation at these nodes, with the goal of reducing the overall job completion time. Our proposed auction also has the desired incentive compatibility property that ensures that mobile devices truthfully reveal their capabilities and costs and that those devices benefit from the task allocation. To deal with node mobility, we perform multiple auctions over adaptive time intervals. We develop a heuristic approach to dynamically find the best time intervals between auctions to minimize unnecessary auctions and the accompanying overheads. We evaluate our framework and methods using both real world and synthetic mobility traces. Our evaluation results show that our game theoretic framework improves the job completion time by a factor of 2-5 in comparison to the time taken for executing the job locally, while minimizing the number of auctions and the accompanying overheads. Our approach is also profitable for the nearby nodes that execute the distributor's tasks with these nodes receiving a compensation higher than their actual costs.

==> otherissues.tex <==
\section{Other Issues of the game theoretic framework}\label{secotherissues}
1-related tasks, general framework, both quality and cost\\
2-undividable tasks\\
3-payment \\
4-collusion, and distributor act cooperatively\\ 

==> systemmodel.tex <==
\section{System Model}\label{secsysmodel}
% no \IEEEPARstart
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)

We consider mobile cloud computing in the presence of selfish smart phones. We assume that all smart phones act rationally and selfishly, and their main goal is to maximize their own profits, not to harm others. There is a distributor node that wants to offload a compute job, with a total work load of $D$ units, to its nearby nodes with the goal of reducing the overall job completion time. Since a smart phone incurs a cost (in form of resource and battery usage) while performing a task on behalf of the distributor, it may not be willing to participate unless the distributor provides right incentives.

We propose a multidimensional auction to model the  job/task allocation in mobile cloud computing. In our auction, the distributor holds the auction among $n$ nearby smart phones called \textit{players}. Each player $i$ has an individual private value $t_i$ called its \textit{type} which consists of the following two parameters:

\begin{itemize}

\item $s_i$: the committed service quotient that player $i$ can provide. In distributed computing applications such as speech to text conversion, the service quotient is related to the amount of data that the smart phone can process in a given time (the smart phone finds this information by estimating its maximum execution time running synthetic benchmark and its energy consumption using techniques like PowerBooter~\cite{powerbooter}). In our system, $s_i$ denotes the amount of data that player $i$ can process per second. It should be noted that the distributor is not aware of the actual $s_i$s until the tasks are completed and the results are received from nearby players who have been assigned the tasks.

\item $c_i$: the cost of player $i$ for performing the task with the committed service quotient. $c_i$ is a function of the committed service quotient, $s_i$, and the player's private cost of performing the task, $\theta_i$. We bound $\theta_i$ such that $0<\theta_{min}\leq\theta_{max}<\infty$. $\theta_i$ is affected by various parameters such as processor speed, available storage, remaining battery level, communication cost, etc. $c_i$ is an increasing function of both $s_i$ and $\theta_i$, and is private information of the player $i$, hence, no one else can determine the exact value of $c_i$.
%Also, $\theta_i \in [\theta_{min}, \theta_{max}]$ and %$0<\theta_{min}\leq\theta_{max}<\infty$. %We model %$c_i(b_i, \theta_i)=s_i\theta_i$.

\end{itemize}

Our mechanism works as follows. First, the distributor sends a probe message to find the nearby nodes. Then, each nearby node $i$, interested in participating, replies by announcing its bid $(c_i, s_i)$. Note that $(c_i, s_i)$ announced by the node $i$ need not be the actual private value of its type, $t_i$. Based on the received bids, the distributor selects a set of players and assigns the tasks to them in proportion to their committed service quotient. To provide incentive to the players for their resources, the distributor compensates them by paying the players. Thus, the distributor must determine payments it must make to the selected players. We assume that the distributor has a budget limit $B$ units that specifies the maximum amount that the distributor can pay for processing one unit of data per second. Each player's utility is defined as total received payment its receives minus its cost of participation.

%A type vector $t = (t_1, t_2, \ldots, t_n)$ comprising all players' types is called \textit{profile}. Given a reported profile, the auction mechanism determines the allocation rule as well as the payments to each player. Each player's utility is defined as its total received payment minus its cost of participation.

%The mechanism works as follows. First, the distributor sends a probe message to find the nearby nodes. Then, the nearby nodes reply by announcing their bids (i.e. $(c_i, s_i)$s). Based on the received bids, the distributor selects a set of players and assigns the tasks to them in proportion to their committed service quotient. To provide incentive for selfish players to act cooperatively, the distributor pays them in compensation. Thus, the distributor should also determine payments to the selected players. We assume that there is a budget limit $B$ that specifies the maximum amount that the distributor can pay for processing one unit of data per second.

Our mechanism implements truthfulness in \textit{dominant equilibrium} implying that each player's best strategy, regardless of other players strategies, is to bid truthfully (i.e. to report actual values of $s_i$ and $c_i$). We prove this desired truthfulness property in Section~\ref{subsecproofs}. Table~\ref{tblnotation} summarizes the notation we use in this and the subsequent sections.

